Breaking the Pre-Planning Barrier: Adaptive Real-Time Coordination of Heterogeneous UAVs

Unmanned Aerial Vehicles (UAVs) offer significant potential in dynamic, perception-intensive tasks such as search and rescue and environmental monitoring; however, their effectiveness is severely restricted by conventional pre-planned routing methods, which lack the flexibility to respond in real-time to evolving task demands, unexpected disturbances, and localized view limitations in real-world scenarios. To address this fundamental limitation, we introduce a novel multi-agent reinforcement learning framework named \textbf{H}eterogeneous \textbf{G}raph \textbf{A}ttention \textbf{M}ulti-agent Deep Deterministic Policy Gradient (HGAM), uniquely designed to enable adaptive real-time coordination between mission UAVs (MUAVs) and charging UAVs (CUAVs). HGAM specifically addresses the previously unsolved challenge of enabling precise, decentralized continuous-action coordination solely based on local, heterogeneous graph-based observations. Extensive simulations demonstrate that HGAM substantially surpasses existing methods, achieving, for example, a 30\% improvement in data collection coverage and a 20\% increase in charging efficiency, providing crucial insights and foundations for the future deployment of intelligent, flexible UAV networks in complex, dynamic environments.

==> sec/2_Background.tex <==
\section{Background}
\label{sec:Background}


\subsection{Partially Observable Markov Decision Process (POMDP)}
Real-world multi-agent scenarios, such as heterogeneous UAV coordination, commonly involve uncertainty and incomplete observations due to limited sensor ranges and dynamic environments. Such scenarios can be rigorously modeled using a Partially Observable Markov Decision Process (POMDP)~\cite{ghosh2021generalization}. Formally, a POMDP extends the Markov Decision Process (MDP) framework and is defined by the tuple \((S, A, T, R, \Omega, O, \gamma)\). At each timestep \(t\), an agent \(i\) receives only a partial observation \(o_t^i \in O\) derived from the global state \(s_t \in S\), and accordingly selects an action \(a_t^i \in A\) following a policy \(\pi_i\), where \(a_t^i \sim \pi_i(\cdot | o_t^i; \theta)\). The global environment then transitions to a new state \(s_{t+1}\) according to the transition probability function \(T(s_{t+1} | s_t, \mathbf{a_t})\), influenced collectively by the actions \(\mathbf{a_t}\) of all participating agents. Each agent subsequently receives a reward \(r_t^i \in R\), guiding future decisions. Observations for the next state are provided through the observation function \(\Omega(o_{t+1} | s_{t+1}, \mathbf{a_t})\), characterizing each agent’s partial information about the environment. The primary objective in solving a POMDP is to find optimal policies that maximize the expected cumulative discounted reward:
\[
\mathbb{E}\left[\sum_{t=0}^{\infty} \gamma^t r_t\right],
\]
where \(\gamma \in [0, 1)\) is the discount factor, balancing immediate versus future rewards. In our context, UAVs must continuously optimize their decisions under limited local observations, aligning perfectly with the POMDP framework.

\subsection{Multi-Agent Deep Deterministic Policy Gradient (MADDPG)}
To address continuous action spaces and cooperative decision-making, multi-agent reinforcement learning algorithms leverage advanced actor-critic architectures. Deep Reinforcement Learning (DRL) methods can be categorized into two main paradigms: value-based approaches, such as Q-learning and Deep Q-Networks (DQN), which optimize the state-action value function \(Q(s,a)=\mathbb{E}[R]\), and policy-based methods, like REINFORCE~\cite{sutton1999policy}, which directly optimize the policy \(\pi\) by maximizing \(J(\theta^\mu)=\mathbb{E}[R]\). Actor-critic methods~\cite{konda1999actor} integrate the strengths of both paradigms, employing an actor that generates actions based on the current policy and a critic that evaluates these actions through value estimation.

Deep Deterministic Policy Gradient (DDPG)~\cite{lillicrap2019continuouscontroldeepreinforcement} extends the actor-critic structure to handle continuous action spaces. In DDPG, the actor network outputs deterministic actions rather than probability distributions, and the critic approximates the Q-function for continuous state-action spaces. To ensure stable training, DDPG employs target networks and exploration noise, often realized through the Ornstein-Uhlenbeck process~\cite{uhlenbeck1930theory}. 

MADDPG further generalizes DDPG to multi-agent environments by assigning each agent an independent actor network \(\mu_i(o_i;\theta_i)\), responsible for making decisions based solely on local observations. Meanwhile, each agent's critic network \(Q_i(\mathbf{o},\mathbf{a};\theta_i)\) centrally evaluates the global value function using all agents’ observations and actions. This centralized-training-decentralized-execution (CTDE) paradigm effectively mitigates non-stationarity in multi-agent settings. The critics are updated by minimizing the Temporal Difference (TD) loss:
\[
\mathcal{L}(\theta_i) = \mathbb{E}\left[\left(y_i - Q_i(\mathbf{o}, \mathbf{a};\theta_i)\right)^2\right],
\]
thus enhancing each agent's decision-making consistency. This architecture particularly suits UAV coordination tasks requiring distributed action selection and centralized evaluation, as in our scenario.

\subsection{Graph Attention Networks (GAT)}
Effective information exchange among heterogeneous agents is critical for cooperative decision-making in complex, partially observable environments. Graph Attention Networks (GAT)~\cite{velivckovic2017graph} offer a powerful solution to model relational structures among agents, dynamically assigning attention to critical neighbors based on relevance. Specifically, GATs aggregate node information via self-attention mechanisms, enhancing the expressive capability to model diverse interactions within heterogeneous groups.

Formally, given a node \(i\), a GAT layer computes its representation \(h_i^l\) by adaptively aggregating information from neighboring nodes \(j\in\mathcal{N}(i)\) according to attention weights \(\alpha_{ij}^l\):
\[
h_i^l = \sigma\left(\sum_{j\in\mathcal{N}(i)}\alpha_{ij}^l W^l h_j^l\right),
\]
where \(\sigma\) denotes a nonlinear activation function (e.g., ELU), \(W^l\) represents learnable weight matrices, and \(\alpha_{ij}^l\) quantifies the importance of node \(j\) to node \(i\). The attention coefficients are obtained via:
\[
\alpha_{ij}^l=\frac{\exp\left(\text{LeakyReLU}(a^l\cdot[W^lh_i^l||W^lh_j^l])\right)}{\sum_{k\in\mathcal{N}(i)}\exp\left(\text{LeakyReLU}(a^l\cdot[W^lh_i^l||W^lh_k^l])\right)},
\]
enabling each node to selectively emphasize essential relationships. Figure~\ref{fig:gat} illustrates a heterogeneous GAT architecture, highlighting how distinct node types (e.g., MUAVs and CUAVs) are integrated through attention-based message passing.

In multi-UAV coordination scenarios like ours, GAT naturally captures dynamic communication and cooperation patterns, significantly improving decision-making by leveraging localized relational structures. Thus, incorporating GAT with MADDPG within our proposed framework allows agents to optimize cooperation dynamically and adaptively, addressing both partial observability and heterogeneity inherent to real-world UAV missions.

